Improving Accuracy in Cell-Perturbation Experiments by Leveraging Auxiliary Information

Modern cell-perturbation experiments expose cells to panels of hundreds of stimuli, such as cytokines or CRISPR guides that perform gene knockouts. These experiments are designed to investigate whether a particular gene is upregulated or downregulated by exposure to each treatment. However, due to high levels of experimental noise, typical estimators of whether a gene is up- or down-regulated make many errors. In this paper, we make two contributions. Our first contribution is a new estimator of regulatory effect that makes use of Gaussian processes and factor analysis to leverage auxiliary information about similarities among treatments, such as the chemical similarity among the drugs used to perturb cells. The new estimator typically has lower variance than unregularized estimators, which do not use auxiliary information, but higher bias. To assess whether this new estimator improves accuracy (i.e., achieves a favorable trade-off between bias and variance), we cannot simply compute its error on heldout data as ``ground truth'' about the effects of treatments is unavailable. Our second contribution is a novel data-splitting method to evaluate error rates. This data-splitting method produces valid error bounds using ``sign-valid'' estimators, which by definition have the correct sign more often than not. Using this data-splitting method, through a series of case studies we find that our new estimator, which leverages auxiliary information, can yield a three-fold reduction in type S error rate.

==> old/junk.tex <==

% For the purposes of this paper, it will be helpful to view a Kronecker product $A \otimes B$ as a linear operator which acts on matrices by modifying the rows according to $A$ and the columns according to $B$.  Specifically, for any matrices $A \in \mathbb{R}^{n_1 \times m_1}$ and $B\in \mathbb{R}^{n_2 \times m_2}$ the Kronecker product $(A\otimes B)$ can be understood as a linear operator on the space of $m_1 \times m_2$  matrices defined by
% \[
% ((A \otimes B)Z)_{i,j} = \sum_k \sum_\ell A_{ik} B_{j\ell} Z_{k\ell}.
% \]
% This point of view also extends to third-order tensors such as $X \in \mathbb{R}^{R \times P \times G}$.  For any triple of matrices $A \in \mathbb{R}^{R' \times R}$, $B \in \mathbb{R}^{P' \times P}$, and $C \in \mathbb{R}^{G' \times G}$, the Kronecker product $A\otimes B \otimes C$ may be viewed as the linear operator on the space of $R\times P \times G$ tensors such that
% \[
% ((A \otimes B\otimes C)X)_{r',p',g'} = \sum_{r,p,g} A_{r',r}B_{p',p}C_{g',g} X_{r,p,g}.
% \]
% To articulate statements about Kronecker products it is helpful to introduce a notation for the basis of vector spaces.  We take $\mathbb{I}$ to denote the indicator function and $\basisvec{N}{i}$ to denote the matrix in $\mathbb{R}^{N\times 1}$ with $\basisvecfull{N}{i}{j}= \mathbb{I}_{i = j}$.  Thus, for example, we may compute that $(\basisvec{P}{p}^\top \otimes \basisvec{G}{g}^\top) \theta = \theta_{p,g}$---though it is important to note that this equality is only well-defined because we may identify the tensor space $\mathbb{R}^{1 \times 1}$ with $\mathbb{R}$.  The statement $\mathrm{cov}(\theta)=K\otimes \Psi$ can thus be understood to signify that 
% \begin{align*}
% \mathrm{cov}(\theta_{p,g},\theta_{p',g'})
% &=(\basisvec{P}{p}^\top \otimes \basisvec{G}{g}^\top) \mathrm{cov}(\theta) (\basisvec{P}{p'} \otimes \basisvec{G}{g'})\\
% &= (\basisvec{P}{p}^\top \otimes \basisvec{G}{g}^\top) (K \otimes \Psi)(\basisvec{P}{p'} \otimes \basisvec{G}{g'}) = K_{p,p'} \Psi_{g,g'}
% \end{align*}

For example, the rows of $\theta \in \mathbb{R}^{P \times G}$ are independent if and only if the covariance of $\theta$ can be expressed as a sum of the form
\[
\sum_p (\basisvec{P}{p} \basisvec{P}{p}^\top)\otimes A_p
\]
for some collection of matrices $A_1,\ldots,A_P$ with $A_p\in \mathbb{R}^{G \times G}$ for each $p$.  This can be verified directly, as such a covariance implies that
\[
\mathrm{cov}(\theta_{p,g},\theta_{p',g}) = \sum_p \mathbb{I}_{p=p'} (A_p)_{g,g'}
\]
will be zero unless $p=p'$.
